On Data Engineering for Scaling LLM Terminal Capabilities

Despite rapid recent progress in the terminal capabilities of large language models, the training data strategies behind state-of-the-art terminal agents remain largely undisclosed. We address this gap through a systematic study of data engineering practices for terminal agents, making two key contributions: (1) Terminal-Task-Gen, a lightweight synthetic task generation pipeline that supports seed-based and skill-based task construction, and (2) a comprehensive analysis of data and training strategies, including filtering, curriculum learning, long context training, and scaling behavior. Our pipeline yields Terminal-Corpus, a large-scale open-source dataset for terminal tasks. Using this dataset, we train Nemotron-Terminal, a family of models initialized from Qwen3(8B, 14B, 32B) that achieve substantial gains on Terminal-Bench 2.0: Nemotron-Terminal-8B improves from 2.5% to 13.0% Nemotron-Terminal-14B improves from 4.0% to 20.2%, and Nemotron-Terminal-32B improves from 3.4% to 27.4%, matching the performance of significantly larger models. To accelerate research in this domain, we open-source our model checkpoints and most of our synthetic datasets at https://huggingface.co/collections/nvidia/nemotron-terminal.

==> sections/1_introduction.tex <==
\section{Introduction}\label{sec::intro}

Physical AI definition.

Contrast document / Math AI with physical AI. We are not trying to solve Physics problems but training models for physical ai.

Focus on capabilities, not processes~\citep{morrisposition}. Common sense that are essential for physical ai capabilities.


==> sections/6_benchmark.tex <==
\section{Introduction}\label{sec::benchmark}

Hello, benchmarking here.
\input{tables/6_benchmark/tbl_common_sense}

==> tables/6_benchmark/tbl_common_sense.tex <==

\begin{table}[h]
    \setlength{\tabcolsep}{4.7pt}
    \small
    \captionsetup{justification=centering}
    \caption{
        Quantitative comparison of post-trained WFM with camera control.
    }
    \centering
    \vspace{-1em}
    \setlength{\tabcolsep}{6pt}
    \begin{tabular}{rccccc}
        \toprule
        & \multicolumn{3}{c}{\bf Camera Trajectory Alignment} & \multicolumn{2}{c}{\bf Video Generation Quality} \\
        \cmidrule(r){2-4} \cmidrule(r){5-6}
        & Pose estimation & Rotation & Translation & \multirow{2}{*}{~~~~ FID $\downarrow$} & \multirow{2}{*}{FVD $\downarrow$} \\
        Method & success rate (\%) $\uparrow$ & error ($\degree$) $\downarrow$ &  error $\downarrow$ & & \\
        \midrule
        CamCo~\citep{xu2024camco} & 43.0\% & 8.277 & 0.185 & ~~~~ 57.49 & 433.24 \vspace{2pt} \\
        \diffusionsevenbvideotoworld- & \multirow{2}{*}{\bf 82.0\%} & \multirow{2}{*}{\bf 1.646} & \multirow{2}{*}{\bf 0.038} & \multirow{2}{*}{~~~~ \bf 14.30} & \multirow{2}{*}{\bf 120.49} \\
        Sample-CameraCond & & & & & \\
        \bottomrule
    \end{tabular}
    \label{tab:camera-results}
\end{table}

